Large $N$ limit of irreducible tensor models: $O(N)$ rank-$3$ tensors with mixed permutation symmetry

It has recently been proven that in rank three tensor models, the anti-symmetric and symmetric traceless sectors both support a large $N$ expansion dominated by melon diagrams [arXiv:1712.00249 [hep-th]]. We show how to extend these results to the last irreducible $O(N)$ tensor representation available in this context, which carries a two-dimensional representation of the symmetric group $S_3$. Along the way, we emphasize the role of the irreducibility condition: it prevents the generation of vector modes which are not compatible with the large $N$ scaling of the tensor interaction. This example supports the conjecture that a melonic large $N$ limit should exist more generally for higher rank tensor models, provided that they are appropriately restricted to an irreducible subspace.

==> preamble.tex <==

%\usepackage{hyperref}
\usepackage{amsfonts,amssymb,amsmath,exscale,bbm}
\usepackage{footnpag} % Footnotes start with 1 at each page
\usepackage[all,knot]{xy}  % xy diagrams
\usepackage{color}
%\usepackage{tikz} 
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{subfig}
\usepackage{enumerate}
%\usepackage{stmaryrd}

%\usepackage[backend=biber]{biblatex}
\usepackage{bbold}

%% formatting
%\setlength{\topmargin}{0pt}
%\setlength{\textheight}{8in}
%\setlength{\textwidth}{6in}
%%\setlength{\parskip}{1.5ex}
%\setlength{\oddsidemargin}{.25in}
%\setlength{\evensidemargin}{0pt}
%%\setlength{\parindent}{0pt}
%\setlength{\baselineskip}{1ex}

% environments



\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{psfrag}
\usepackage{array}
\usepackage{bbm}
%\usepackage{hyperref}
\usepackage{amsthm}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}

\oddsidemargin 0.0cm
\evensidemargin 0.0cm
\topmargin 0cm
\textwidth 16.5cm
\setlength{\textheight}{22cm}

\newcommand{\f}{\frac}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\rar}{\rightarrow}
\newcommand{\pd}{\partial}

% Calligraphic letters
%----------------------
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cZ}{{\mathcal Z}}


\newcommand{\sK}{{\cal K}}
\newcommand{\sF}{{\cal F}}
\newcommand{\sP}{{\cal P}}
\newcommand{\sT}{{\cal T}}
\newcommand{\sE}{{\cal E}}
\newcommand{\sH}{{\cal H}}
\newcommand{\sL}{{\cal L}}
\newcommand{\sI}{{\cal I}}
\newcommand{\sB}{{\cal B}}
\newcommand{\sS}{{\cal S}}
\newcommand{\sV}{{\cal V}}
\newcommand{\sN}{{\cal N}}
\newcommand{\sD}{{\cal D}}
\newcommand{\sh}{{\cal h}}

\newcommand{\g}{{\mathfrak{g}}}
\newcommand{\mH}{{\mathfrak{h}}}
\newcommand{\Inv}{{\mathrm{Inv}}}




% Inverse element

\def\inv{{\mbox{\tiny -1}}}
\def\minus{{\mbox{\small -}}}
\def\plus{{\mbox{\tiny +}}}
\newcommand\unit{\mathbbm{1}}


% fancy letter

\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}

\newcommand{\fa}{\mathbb{a}}
\newcommand{\fb}{\mathbb{b}}
\newcommand{\fc}{\mathbb{c}}
\newcommand{\fd}{\mathbb{d}}
\newcommand{\fe}{\mathbb{e}}
\newcommand{\ff}{\mathbb{f}}
\newcommand{\fg}{\mathbb{g}}

\newcommand{\es}{{e^*}}
\newcommand{\vs}{{v^*}}
\newcommand{\fs}{{f^*}}

\newcommand{\id}{\mathbb{I}}

\newcommand\beq{\begin{equation}}
\newcommand\eeq{\end{equation}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bes}{\begin{eqnarray}}
\newcommand{\ees}{\end{eqnarray}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\mone}{^{\minus 1}}

\def\bfR{{\bf R}}
\def\bfu{{\bf u}}
\def\bfa{{\bf a}}
\def\bfx{{\bf x}}
\def\bfg{{\bf g}}
\def\bfe{{\bf e}}
\def\bfT{{\bf T}}
\def\hPhi{{\hat \Phi}}
\def\hPsi{{\hat \Psi}}
\def\tf{\tilde f}
\def\tPhi{{\tilde \Phi}}
\def\tPsi{{\tilde \Psi}}
\def\psibar{\overline{\psi}}
\def\dia{\diamond}
\def\st{\divideontimes}
\def\ov{\overline}
\def\kap{\kappa'}
\def\f{\frac} \def\t{\textrm{Tr}} \def\MP{M_P}
\def\dag{^\dagger}
\def\tl{\widetilde}
\def\tdelta{\tl{\delta}}
\def\arr{\rightarrow}
\def\eps{\epsilon}
\def\pp{\partial}
\def\ka{\kappa}
\def\cc{{\cal C}}
\def\la{\langle}
\def\ra{\rangle}
\def\ot{{\,\otimes \,}}
\def\poi#1{\{ #1 \}}
\def\com#1{[ #1 ]}
\def\act{\rhd}
\def\mn{{\mu\nu}}
\def\vphi{{\varphi}}
\def\vphib{\overline{{\varphi}}}
\def\Jb{\overline{J}}
\def\tvphi{{\tilde \varphi}}
\def\tF{{\tilde F}}
\def\g{\mathfrak{g}}
\def\tg{\tilde{g}}
\def\tu{\tilde{u}}
\def\demi{\frac{1}{2} }
\def\ie{{i.e. \/}}
\def\eg{{e.g. \/}}
\def\cf{{c.f. \/}}
\def\dr{{\rightarrow}}
\newcommand{\one}{\mbox{$1 \hspace{-1.0mm}  {\bf l}$}}
\def\cop{{\bigtriangleup}}
\def\aste{{\divideontimes}}
\def\Phib{\overline{\Phi}}
\def\omegab{\overline{\omega}}
\def\tS{\widetilde{S}}
\def\tC{\widetilde{C}}
\def\tu{\tilde{u}}
\def\tt{\tilde{t}}

\def\aa{{\cal A}} \def\bb{{\cal B}} \def\cc{{\cal C}} \def\dd{{\cal D}} \def\Ee{{\cal E}} \def\ff{{\cal F}} \def\ggg{{\cal G}}
\def\hh{{\cal H}} \def\ii{{\cal I}} \def\jj{{\cal J}} \def\kk{{\cal K}} \def\lll{{\cal L}} \def\mm{{\cal M}} \def\nn{{\nonumber}}
\def\oo{{\cal O}} \def\ppp{{\cal P}} \def\qq{{\cal Q}} \def\rr{{\cal R}} \def\ss{{\cal S}} \def\tt{{\cal T}} \def\uu{{\cal U}}
\def\vv{{\cal V}} \def\ww{{\cal W}} \def\xx{{\cal X}} \def\yy{{\cal Y}} \def\zz{{\cal Z}}
\def\tr{{\mathrm{tr}}}

\def\dg{{\dd (G)}}
\def\hphi{{\widehat \phi}}
\def\hvpsi{{\widehat \psi}}
\def\hpsi{{\widehat \psi}}
\def\tstar{{\, \bullet\,}}
\def\ttstar{{\, \star\,}}
\def\tttstar{{\, * \, }}
\def\bicross{{\blacktriangleright\hspace{-1.75mm}\lhd }}
\def\bltimes{{>\hspace{-1.0mm} \blacktriangleleft}}
\def\coact{{\, \triangleleft \, }}
\def\coactb{{\, \blacktriangleright \, }}
\def\act{{\, \triangleright\, }}
\def\brtimes{{\blacktriangleright\hspace{-1.0mm}< }}
\def\rltimes{{\,\triangleright\hspace{-1.4mm}< \,}}
\def\lltimes{{\,>\hspace{-1.4mm} \triangleleft\,}}
\def\double{{\triangleright\hspace{-0.5mm}\triangleleft}}

\def\tLambda{\tl{\Lambda}}
\newcommand{\su}{\mathfrak{su}}
\newcommand{\an}{\mathfrak{an}}
\newcommand{\so}{\mathfrak{so}}
\newcommand{\SU}{\mathrm{SU}}
\newcommand{\AN}{\mathrm{AN}}
\newcommand{\U}{\mathrm{U}}
\newcommand{\ISU}{\mathrm{ISU}}
\newcommand{\Sp}{\mathrm{Sp}}
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\mO}{\mathrm{O}}
\newcommand{\SL}{\mathrm{SL}}
\newcommand{\sll}{\mathrm{sl}}
\newcommand{\ISO}{\mathrm{ISO}}
\newcommand{\Spin}{\mathrm{Spin}}
\newcommand{\isu}{\mathfrak{isu}}
\newcommand{\mat}[2]{\left(\begin{array}{#1} #2\end{array}\right)}
\def\kkk{{\mathfrak{k}}}
\def\dsu{{\dd(\SU(2))}}
\def\csu{{\cc(\SU(2))}}
\def\tdelta{{\tilde\delta}}
\def\extd{\mathrm {d}}
\newcommand{\e}{\epsilon}
\def\tphi{{ \tilde\phi}}
\def\hfrak{{\mathfrak{h}}}


% operations

%\newcommand\tensor{\otimes}
\newcommand\To{\Rightarrow}
\newcommand{\im}{\mathrm{im}}
\newcommand{\iso}{\cong}

\newcommand\acts\triangleright


% lists
\newcounter{letter} \newcounter{numeral} \newcounter{Numeral}

\newenvironment{alphalist}{
\begin{list}{(\alph{letter})}{\usecounter{letter}}
}{\end{list}}

\newenvironment{Alphalist}{
\begin{list}{(\Alph{letter})}{\usecounter{letter}}
}{\end{list}}

\newenvironment{Romanlist}{
\begin{list}{\Roman{Numeral}}{\usecounter{Numeral}}
}{\end{list}}

\newenvironment{romanlist}{
\begin{list}{(\roman{numeral})}{\usecounter{numeral}}
}{\end{list}}


% other macros
%\newcommand\arr{\longrightarrow}
\renewcommand\d{\partial}
\newcommand\vp{\vec{p}}
\newcommand\bchi{\overline{\chi}}
\newcommand\Tr{\mathrm{Tr}}
\def\vphi{\varphi}
\def\vphihat{\widehat{\varphi}}
\def\tvphihat{\widehat{\tilde{\varphi}}}
\def\tpsi{\tilde{\psi}}
\def\hvphi{\widehat{\varphi}}
\def\fhat{\widehat{f}}
\def\hhat{\widehat{h}}
\def\e{\mbox{e}}
\def\extd{\mathrm {d}}
\def\ve{\varepsilon}
\def\bbar{ \overline{b}}


% functions
\newcommand\maps{\colon}

% theorems and proofs

\newtheorem{theo}{Theorem}%[section]
\newtheorem{lemma}[theo]{Lemma}
\newtheorem{prop}[theo]{Proposition}
\newtheorem{defn}[theo]{Definition}
\newtheorem{cor}[theo]{Corollary}

\newcommand{\comment}[1]{{{\footnotesize{\color{magenta} #1}}}}
\newcommand{\comf}[1]{{{\footnotesize{\color{blue} #1}}}}
\def\C{{\mathbbm C}}
\def\N{{\mathbbm N}}
\def\Z{{\mathbbm Z}}
\def\R{{\mathbbm R}}


\newcommand{\cexG}{\mathcal G_{\text{color}}}
\newcommand{\bJ}{ J_{\partial} }


\newcommand{\prf }{\medskip\noindent{\bf Proof\ }}



\newcommand{ \colred }{ \color{red}}



%%%%%%%%%%%%%%
%%
